FcaNet: Frequency Channel Attention Networks

Attention mechanism, especially channel attention, has gained great success in the computer vision field. Many works focus on how to design efficient channel attention mechanisms while ignoring a fundamental problem, i.e., channel attention mechanism uses scalar to represent channel, which is difficult due to massive information loss. In this work, we start from a different view and regard the channel representation problem as a compression process using frequency analysis. Based on the frequency analysis, we mathematically prove that the conventional global average pooling is a special case of the feature decomposition in the frequency domain. With the proof, we naturally generalize the compression of the channel attention mechanism in the frequency domain and propose our method with multi-spectral channel attention, termed as FcaNet. FcaNet is simple but effective. We can change a few lines of code in the calculation to implement our method within existing channel attention methods. Moreover, the proposed method achieves state-of-the-art results compared with other channel attention methods on image classification, object detection, and instance segmentation tasks. Our method could consistently outperform the baseline SENet, with the same number of parameters and the same computational cost. Our code and models will are publicly available at https://github.com/cfzd/FcaNet.

==> tables/frequency_combination.tex <==

\begin{table}[htbp]
	\centering
	\caption{The results of using different numbers of frequency components on ImageNet with ResNet-50 backbone.}
	\label{combination}
	\begin{tabular}{ccc}
		\toprule
		Number    & Top-1 acc   & Top-5 acc  \\
		\midrule
		1   & 77.26     & 93.55\\
		2	& 78.40		& 94.07\\
		4	& 78.38		& 94.03\\
		8   & 78.33		& 94.06\\ 
		16 	& \textbf{78.52}  	& \textbf{94.14}\\
		32 	& 78.42  	& 94.10\\
		\bottomrule
	\end{tabular}
\end{table}



%\begin{table}[htbp]
%	\centering
%	\caption{The effects of different combinations of frequency components on the ImageNet dataset.}
%	\label{combination}
%	\begin{tabular}{ccc}
%		\toprule
%		Number    & Top-1 acc   & Top-5 acc  \\
%		\midrule
%		1   &  & \\
%		2	&  77.30 & 93.51\\
%		4	&  77.27 & 93.57\\
%		8   &  77.51 & 93.63\\ 
%		16 	&  77.17 & 93.53\\
%		32 	&  77.60 & 93.78\\
%		\bottomrule
%	\end{tabular}
%\end{table}

%\begin{table}[htbp]
%	\centering
%	\caption{The effects of different combinations of frequency components on the ImageNet dataset.}
%	\label{combination}
%	\begin{tabular}{ccc}
%		\toprule
%		Number    & Top-1 acc   & Top-5 acc  \\
%		\midrule
%		1   & 77.26 & 93.55\\
%		2	&  78.40 & 94.07\\
%		4	&  78.27 & 94.06\\
%		8   &  78.25 & 94.01\\ 
%		16 	&  78.26 & 94.12\\
%		32 	&  78.37 & 94.08\\
%		\bottomrule
%	\end{tabular}
%\end{table}

==> texs/method.tex <==

\section{Method}

In this section, we first revisit the formulation of channel attention and DCT frequency analysis. Then, based on these works, we elaborate on the derivation of our multi-spectral channel attention framework. Meanwhile, along with the multi-spectral channel attention framework, three kinds of frequency components selection methods are proposed. At last, we give discussions about effectiveness, complexity, and code implementation.

\subsection{Revisiting Channel Attention and DCT}

We first elaborate on the definitions of channel attention mechanism and discrete cosine transform. 
% Then, we briefly summarize the properties of channel attention and DCT.

\label{sec_ca_and_dct}

\paragraph{Channel Attention}
The channel attention mechanism is widely used in CNNs. It uses a learnable network to weight the importance of each channel and generates more informative outputs. Suppose $X \in \mathbb{R}^{C \times H \times W}$ is the image feature tensor in networks, $C$ is the number of channels, $H$ is the height of the feature, and $W$ is the width of the feature. Then the attention mechanism can be written as \cite{hu2018squeeze,wang2020eca}:
\begin{equation}
    att = sigmoid(fc(gap(X))),
    \label{eq_ca}
\end{equation}
where $att \in \mathbb{R} ^ {C}$ is the attention vector, $sigmoid$ is the Sigmoid function, $fc$ represents the mapping functions like fully connected layer or one-dimensional convolution, and $gap$ is the global average pooling. After obtaining the attention vector of all $C$ channels, each channel of input $X$ is scaled by the corresponding attention value:
\begin{equation}
    \widetilde{X}_{:,i,:,:} = att_i X_{:,i,:,:}, \:\:\: s.t. \;\; 
    i \in \{0,1,\cdots,C-1\},
\end{equation}
in which $\widetilde{X}$ is the output of attention mechanism, $att_i$ is the $i$-th element of attention vector, and $X_{:,i,:,:}$ is the $i$-th channel of input.

\paragraph{Discrete Cosine Transform (DCT)}

Typically, the basis function of two-dimensional (2D) DCT \cite{ahmed1974discrete} is:
\begin{equation}
    B_{h,w}^{i,j} = \cos(\dfrac{\pi h}{H}(i+\dfrac{1}{2}))\cos(\dfrac{\pi w}{W}(j+\dfrac{1}{2})).
    \label{eq_basis}
\end{equation}
Then the 2D DCT can be written as:
\begin{equation}
    \begin{aligned}
        &f_{h,w}^{2d}  =  \sum_{i=0}^{H-1} \sum_{j=0}^{W-1} x_{i,j}^{2d} B_{h,w}^{i,j}\\
        s.t. \;\; h \in \{0,1, & \cdots,H-1\}, w \in \{0,1,\cdots,W-1\},
    \end{aligned}
    \label{eq_2ddct}
\end{equation}
in which $f^{2d} \in \mathbb{R}^{H \times W}$ is the 2D DCT frequency spectrum, $x^{2d} \in \mathbb{R}^{H \times W}$ is the input, $H$ is the height of $x^{2d}$, and $W$ is the width of $x^{2d}$. Correspondingly, the inverse 2D DCT can be written as:
\begin{equation}
    \begin{aligned}
        & x_{i,j}^{2d} =  \sum_{h=0}^{H-1} \sum_{w=0}^{W-1} f_{h,w}^{2d} B_{h,w}^{i,j},\\
         s.t. \;\; i \in \{0,1, & \cdots,H-1\}, j \in \{0,1,\cdots,W-1\}.
    \end{aligned}
    \label{eq_2didct}
\end{equation}
Please note that in Eqs.~\ref{eq_2ddct} and \ref{eq_2didct}, some constant normalization factors are removed for simplicity, which will not affect the results in this work.

% With the definitions of channel attention and DCT, we can summarize two key properties: a) existing methods use GAP as their compression before channel attention. b) DCT can be viewed as a weighted sum of inputs with the cosine parts being the weights. 

% GAP is an operation of mean value due to constrained computational overhead, and it can be viewed as the simplest spectrum of input. As described in the introduction section, it is inadequate to use single GAP information in channel attention. Motivated by these properties, we can proceed to introduce our multi-spectral channel attention method.

\subsection{Multi-Spectral Channel Attention}
\label{sec_msca}
In this section, we first theoretically discuss the problem of existing channel attention mechanisms. Based on the theoretical analysis, we then elaborate on the network design of the proposed method.

\paragraph{Theoretical Analysis of Channel Attention}

As discussed in Sec.~\ref{sec_ca_and_dct}, DCT can be viewed as a weighted sum of inputs. We further propose that GAP is actually a special case of 2D DCT.
\begin{theorem}
    GAP is a special case of 2D DCT, and its result is proportional to the lowest frequency component of 2D DCT.
    \label{theo}
\end{theorem}

\begin{figure*}[t]
    \centering
    % \includegraphics[width=0.9\textwidth]{figures/main.pdf}
    \subfigure[Original SENet]{\includegraphics[width=0.93\textwidth]{figures/main_a_v2.pdf}}
    \subfigure[Multi-spectral channel attention]{\includegraphics[width=0.93\textwidth]{figures/mainb_v4.pdf}}
    \caption{Illustration of existing channel attention and multi-spectral channel attention. For simplicity, the 2D DCT indices are represented in the one-dimensional format. We can see that our method uses multiple frequency components with the selected DCT bases, while SENet only uses GAP in channel attention. Best viewed in color.}
    \label{fig_main}
\end{figure*}

\begin{proof} Suppose $h$ and $w$ in Eq.~\ref{eq_2ddct} are $0$, we have:
\begin{equation}
    \begin{aligned}
        f_{\textcolor{red}{0,0}}^{2d} &= \sum_{i=0}^{H-1} \sum_{j=0}^{W-1} x_{i,j}^{2d} \cos(\dfrac{\textcolor{red}{0}}{H}(i+\dfrac{1}{2}))\cos(\dfrac{\textcolor{red}{0}}{W}(j+\dfrac{1}{2}))   \\
        & = \sum_{i=0}^{H-1} \sum_{j=0}^{W-1} x_{i,j}^{2d} \\
        & = gap(x^{2d}) HW.
    \end{aligned}
    \label{eq_proof}
\end{equation}

In Eq.~\ref{eq_proof}, $f_{0,0}^{2d}$ represents the lowest frequency component of 2D DCT, and it is proportional to GAP. In this way, theorem \ref{theo} is proved.
\end{proof}



\paragraph{Multi-Spectral Channel Attention Module}
Based on the theoretical analysis and theorem \ref{theo}, we find the information used in existing channel attention is inadequate, and the compression method GAP of channel attention is a special case of 2D DCT. In this way, we could naturally generalize GAP to more frequency components of 2D DCT and introduce more information to solve the problem of inadequate information in channel attention. 

To introduce more information, we propose to use multiple frequency components of 2D DCT, including the lowest frequency component, i.e., GAP. 



First, the input $X$ is split into many parts along the channel dimension. Denote $[X^0,X^1, \cdots, X^{n-1}]$ as the parts, in which $X^i \in \mathbb{R}^{C' \times H \times W}$, $i \in \{0,1, \cdots, n-1\}$, $C' = \dfrac{C}{n}$, and $C$ should be be divisible by $n$. For each part, a corresponding 2D DCT frequency component is assigned, and the 2D DCT results can be used as the compression results of channel attention. In this way, we have:
\begin{equation}
    \begin{aligned}
        Freq^i & = \text{2DDCT}^{u,v}(X^i),  \\
        & = \sum_{h=0}^{H-1} \sum_{w=0}^{W-1} X_{:,h,w}^i B_{h,w}^{u,v} \\
        & s.t. \;\; i \in \{0,1,\cdots,n-1\},
    \end{aligned}
    \label{eq_2ddct_network}
\end{equation}
in which $[u,v]$ are the frequency component 2D indices corresponding to $X^i$, and $Freq^i \in \mathbb{R}^{C'}$ is the $C'$-dimensional vector after the compression. The whole compression vector can be obtained by concatenation:
\begin{equation}
    Freq = \text{cat}([Freq^0,Freq^1,\cdots,Freq^{n-1}]),
    \label{eq_cat}
\end{equation}
in which $Freq \in \mathbb{R}^C$ is the obtained multi-spectral vector.
The whole multi-spectral channel attention framework can be written as:
\begin{equation}
    ms\_att = sigmoid(fc(Freq)).
    \label{eq_final}
\end{equation}

From Eqs.~\ref{eq_cat} and \ref{eq_final}, we can see that our method generalizes the original method that only uses the GAP, i.e., the lowest frequency component to a framework with multiple frequency sources. By doing so, the inadequate problem of original methods is addressed. The overall illustration of our method is shown in Fig.~\ref{fig_main}.

\paragraph{Criteria for Choosing Frequency Components}
There exists an important problem of how to choose frequency component indices $[u,v]$ for each part $X^i$. In order to fulfill the multi-spectral channel attention, we propose three kinds of criteria, which are FcaNet-LF (Low Frequency), FcaNet-TS (Two-Step selection), and FcaNet-NAS (Neural Architecture Search). 

\textbf{FcaNet-LF} means FcaNet with low-frequency components. As we all know, many compression methods use low-frequency information of DCT to compress information. Moreover, some methods \cite{hu2018squeeze, xu2020learning} have shown CNNs prefer low-frequency information. In this way, the first criterion for choosing frequency components is to only select low-frequency components. 

\textbf{FcaNet-TS} means FcaNet with components selected with a two-step selection. The main idea is to first determine the importance of each frequency component and then determine the effects of using different numbers of frequency components together. First, we examine the results of each frequency component in channel attention individually. Then, we choose the Top-k highest performance frequency components based on the results.

\textbf{FcaNet-NAS} means FcaNet with searched components. For this criterion, we use neural architecture search to search the best frequency component for channels. For each part $X^i$, a set of continuous variables $\alpha=\{\alpha^{(u,v)}\}$ are assigned to search components. The frequency components of this part can be written as:
\begin{equation}
    Freq^i_{nas} = \sum_{\scaleto{(u, v) \in O}{6pt}} \dfrac{\exp(\alpha^{(u,v)})}{ \sum_{\scaleto{(u', v') \in O}{6pt}  } \exp(\alpha^{(u',v')}) } \text{2DDCT}^{u,v}(X^i),
\end{equation}
in which $O$ is the set containing all 2D DCT frequency component indices.
After training, the frequency component is derived by 
$(u^*,v^*) = \argmax_{(u,v) \in O} \{\alpha^{(u,v)}\}$.


The ablation studies about these criteria can be seen in Sec.~\ref{sec_ablation}.

\subsection{Discussion}

\paragraph{How the multi-spectral framework compress and embed more information}
In Sec.~\ref{sec_msca}, we show that only using GAP in channel attention is actually discarding information of all other frequency components except the lowest one, i.e., GAP. In this way, generalizing channel attention in the frequency domain and using the multi-spectral framework could naturally embed more information in the channel attention mechanism. 

Besides the above derivation, we also give a thought experiment to show that more information could be embedded. As we all know, deep networks are redundant \cite{he2017channel,zhuang2018discrimination}. If two channels are redundant for each other, we can only get the same information using GAP. However, in our multi-spectral framework, it is possible to extract more information from redundant channels because different frequency components contain different information. In this way, the proposed multi-spectral framework could embed more information in the channel attention mechanism.

\paragraph{Complexity analysis}
We analyze the complexity of our method from two aspects: the number of parameters and the computational cost.

For the number of parameters, our method has no extra parameters compared with the baseline SENet because the weights of 2D DCT are pre-computed constant.

For the computational cost, our method has a negligible extra cost and can be viewed as having the same computational cost as SENet. With ResNet-34, ResNet-50, ResNet-101, and ResNet-152 backbone, the relative computational cost increases of our method are $0.04\%$, $0.13\%$, $0.11\%$, and $0.11\%$ compared with SENet, respectively. More results can be found in Table~\ref{classification}.

\paragraph{A Few lines of code change}
Another important property of the proposed multi-spectral framework is that it can be easily realized with existing channel attention implementations. The only difference between our method and SENet is the channel compression method (GAP vs. multi-spectral 2D DCT). As described in Sec.~\ref{sec_ca_and_dct} and Eq.~\ref{eq_2ddct_network}, 2D DCT can be viewed as a weighted sum of inputs. It can be simply realized by element-wise multiplication and summation. In this way, our method could be easily integrated into arbitrary channel attention methods.

% \begin{minted}[linenos,framesep=2mm,baselinestretch=1.2,fontsize=\footnotesize]{python}
% from torch import nn
%
% class SELayer(nn.Module):
%     def __init__(self, channel, reduction=16):
%         super(SELayer, self).__init__()
%         self.avg_pool = nn.AdaptiveAvgPool2d(1)
%         self.fc = nn.Sequential(
%             nn.Linear(channel, channel // reduction, 
%             bias=False),
%             nn.ReLU(inplace=True),
%             nn.Linear(channel // reduction, channel, 
%             bias=False),
%             nn.Sigmoid()
%         )
%
%     def forward(self, x):
%         b, c, _, _ = x.size()
%         y = self.avg_pool(x).view(b, c)
%         y = self.fc(y).view(b, c, 1, 1)
%         return x * y.expand_as(x)
%    
% \end{minted}
% \lstset{basicstyle=\tiny,style=mystyle}
% \begin{figure*}
%     \captionsetup{type=lstlisting}
%     \begin{sublstlisting}{0.4\linewidth}
%         \begin{lstlisting}[language=Python]
%             from torch import nn
%
%             class SELayer(nn.Module):
%                 def __init__(self, channel, reduction=16):
%                     super(SELayer, self).__init__()
%                     self.avg_pool = nn.AdaptiveAvgPool2d(1)
%                     self.fc = nn.Sequential(
%                         nn.Linear(channel, channel // reduction, 
%                         bias=False),
%                         nn.ReLU(inplace=True),
%                         nn.Linear(channel // reduction, channel, 
%                         bias=False),
%                         nn.Sigmoid()
%                     )
%            
%                 def forward(self, x):
%                     b, c, _, _ = x.size()
%                     y = self.avg_pool(x).view(b, c)
%                     y = self.fc(y).view(b, c, 1, 1)
%                     return x * y.expand_as(x)
%         \end{lstlisting}
%         \caption{Caption for first listing}
%         \label{lst_se}
%     \end{sublstlisting}
%
%     \begin{sublstlisting}{0.4\linewidth}
%         \begin{lstlisting}[language=Python]
%             from torch import nn
%
%             class SELayer(nn.Module):
%                 def __init__(self, channel, reduction=16):
%                     super(SELayer, self).__init__()
%                     self.avg_pool = nn.AdaptiveAvgPool2d(1)
%                     self.fc = nn.Sequential(
%                         nn.Linear(channel, channel // reduction, 
%                         bias=False),
%                         nn.ReLU(inplace=True),
%                         nn.Linear(channel // reduction, channel, 
%                         bias=False),
%                         nn.Sigmoid()
%                     )
%            
%                 def forward(self, x):
%                     b, c, _, _ = x.size()
%                     y = self.avg_pool(x).view(b, c)
%                     y = self.fc(y).view(b, c, 1, 1)
%                     return x * y.expand_as(x)
%         \end{lstlisting}
%         \caption{Caption for second listing}
%         \label{lst_our}
%     \end{sublstlisting}
%     \caption{General caption for all 3}
%     \label{lst_all}
% \end{figure*}
    
% As we can see in Listings~\ref{lst_se} and~\ref{lst_our}...
